Program Repair for Hyperproperties

We study the repair problem for hyperproperties specified in the temporal logic HyperLTL. Hyperproperties are system properties that relate multiple computation traces. This class of properties includes information flow policies like noninterference and observational determinism. The repair problem is to find, for a given Kripke structure, a substructure that satisfies a given specification. We show that the repair problem is decidable for HyperLTL specifications and finite-state Kripke structures. We provide a detailed complexity analysis for different fragments of HyperLTL and different system types: tree-shaped, acyclic, and general Kripke structures.

==> combined.tex <==
\section{Combined Complexity}
\label{sec:combined}

We now analyze the complexity of the refinement problem in the size of the 
\emph{combined} input, consisting of both the Kripke structure {\em and} the 
HyperLTL formula. Again, we separately focus on trees and acyclic graphs.

\subsection{Trees}

\subsection{Acyclic Kripke Structures}

%\noindent {\bf Instance.} An acyclic Ktipke structure $\krip = \ktuple$ and a 
%HyperLTL formula of the form $\varphi = (\forall^+\exists^+)^k\psi$.\\

%\noindent {\bf Decision problem (AEkTREE-C).} Whether $[\krip \models \varphi] 
%= \top$?

For HyperLTL formulas with bounded quantifier alternation, trees and acyclic 
graphs have the same model checking complexity (except for the special case of 
exactly 
one universal and one existential quantifier). We match the lower bounds for 
trees from Theorem~\ref{thrm:eak-tree} with upper bounds for acyclic graphs.

\begin{theorem}
\label{thrm:aektree-c}
\PR{(EA/AE)k-HyperLTL}{\mbox{acyclic}} is 
\comp{$\mathsf{\Sigma^p_{k+1}}$-complete} in the combined size of the Kripke 
structure and the formula, if the leading quantifier is 
existential and \comp{$\mathsf{\Pi^p_{k+1}}$-complete} if the leading 
quantifier is universal.
\end{theorem}

\begin{proof}
We show membership in \comp{$\mathsf{\Sigma^p_{k+1}}$} and 
\comp{$\mathsf{\Pi^p_{k+1}}$}, respectively, by induction over $k$. For the 
base case, $k = 0$, where  the formula is alternation-free, the refinement 
problem can be solved in \comp{NP} and \comp{co-NP}, respectively, as follows. 
If the quantifiers are existential, we can nondeterministically guess a 
combination of the traces as a refinement and verify the correctness of the 
guess in polynomial time, as the length of each trace is bounded by the number 
of states. Likewise, if the quantifiers are universal, we can universally guess 
a combination of the traces as a refinement and verify the correctness of the 
guess in polynomial time.

For $k+1$ quantifier alternations, suppose that the first quantifier is
existential. Since the Kripke structure is acyclic, the length of the traces is 
bounded by the number of states. We can thus nondeterministically guess the 
existentially quantified traces in polynomial time and verify the correctness 
of the guess, by the induction hypothesis, in \comp{$\mathsf{\Pi^p_{k+1}}$}. 
Hence, the refinement problem for $k+1$ is in \comp{$\mathsf{\Sigma^p_{k+2}}$}. 
Likewise, if the first quantifier is universal, we universally guess the 
universally quantified traces in polynomial time and verify the correctness of 
the guess, by the induction hypothesis, in \comp{$\mathsf{\Sigma^p_{k+1}}$}. 
Hence, the model checking problem for $k+1$ is in 
\comp{$\mathsf{\Pi^p_{k+2}}$}. 

Together with the lower bounds for trees in Theorem~\ref{thrm:eak-tree}, we 
obtain \comp{$\mathsf{\Sigma^p_{k+1}}$/$\mathsf{\Pi^p_{k+1}}$-completeness} for 
$k$ quantifier alternations.

\qed
\end{proof}


